CombiNeRF: A Combination of Regularization Techniques for Few-Shot Neural Radiance Field View Synthesis

Neural Radiance Fields (NeRFs) have shown impressive results for novel view synthesis when a sufficiently large amount of views are available. When dealing with few-shot settings, i.e. with a small set of input views, the training could overfit those views, leading to artifacts and geometric and chromatic inconsistencies in the resulting rendering. Regularization is a valid solution that helps NeRF generalization. On the other hand, each of the most recent NeRF regularization techniques aim to mitigate a specific rendering problem. Starting from this observation, in this paper we propose CombiNeRF, a framework that synergically combines several regularization techniques, some of them novel, in order to unify the benefits of each. In particular, we regularize single and neighboring rays distributions and we add a smoothness term to regularize near geometries. After these geometric approaches, we propose to exploit Lipschitz regularization to both NeRF density and color networks and to use encoding masks for input features regularization. We show that CombiNeRF outperforms the state-of-the-art methods with few-shot settings in several publicly available datasets. We also present an ablation study on the LLFF and NeRF-Synthetic datasets that support the choices made. We release with this paper the open-source implementation of our framework.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage{comment}
%\usepackage[dvipsnames]{xcolor}
\usepackage[table]{xcolor}
\usepackage{makecell}
\usepackage{stmaryrd}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

==> sec/0_abstract.tex <==
\begin{abstract}
\begin{comment}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{comment}
Neural Radiance Field (NeRF) has shown impressive results for novel view synthesis when a sufficiently large amount of views are available. When dealing with sparse input views, hence having much less information of the scene, the training could overfit to those input views, leading the resulting rendering to artifacts and inconsistencies over the geometry and color, especially with few-shot setting. Regularization is a valid solution that helps NeRF generalization. Our idea is that the combination of different forms of regularization can lead to better quality renderings because, singularly, they act for a specific problem but together the benefits adds up.

With the knowledge of some forms of regularization in the literature, we combine (Combi-NeRF) them, applying some changes with respect to the original implementations.
\begin{comment}
We consider an information-theoretic approach that includes a regularization of neighboring rays distributions, then a smoothness term is adopted to regularize near geometries and we regularize single ray distribution in order to have a specific hitting point on the scene, that reflects real world scenarios.
\end{comment}
We regularize single and neighboring rays distribution and a smoothness term is adopted to regularize near geometries.
After these geometric approaches, we focused on Lipshitz function and also on input features regularization of the network. We provide an unified and unique implementation that includes all these regularization techniques.

We show that our implementation outperforms the state-of-the-art methods with few shot settings, including the LLFF and NeRF-synthetic dataset, obtaining better quality reconstructions. We also ablate the contribution of the components of our implementation considering both LLFF and Nerf-synthetic dataset.

Our code is available in (link github Combi-NeRF).
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
\begin{figure}[t] \centering
    \makebox[0.11\textwidth]{Vanilla}
    \makebox[0.11\textwidth]{}
    \makebox[0.11\textwidth]{Combi-NeRF}
    \makebox[0.11\textwidth]{}
    \\
    \includegraphics[width=0.11\textwidth]{images/trex/ngp_ep1667_0003_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/Vanilla/trex/ngp_ep1667_0003_rgb.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/trex/ngp_ep1667_0003_depth.png}
    \includegraphics[width=0.11\textwidth]{images/Vanilla/trex/ngp_ep1667_0003_depth.png}
    \caption{NeRF struggles on few-shot settings. It's shown T-rex scenario with 6-view setting.} 
    \label{fig:figure0}
\end{figure}
Neural Radiance Fields \cite{NeRF} has emerged as a powerful approach for scene reconstruction and photorealistic rendering from sparse 2D images. By leveraging neural networks to model the volumetric scene representation, NeRF can generate high-quality novel views of scenes.
As the MLP networks are queried multiple times for each pixel to be rendered, a lightweight architecture allows to dramatically speed up the whole rendering pipeline.
Multiresolution hash encoding, proposed in \cite{Instant-NGP}, allows for enhancing the efficiency and speed of scene reconstruction by employing a shallow MLP with no reported visual accuracy loss.
However, to achieve high accuracy in its predictions and avoid artifacts, NeRF often relies on a large number of images, which can be impractical in real-world scenarios. 

Regularization is crucial for improving the visual fidelity of rendered images, ensuring more coherent predictions. Several works \cite{Reg-NeRF, Info-NeRF, Mip-NeRF360, DiffusioNeRF} proposed to constrain the MLP network during training by adding term losses. 
Lipshitz regularization \cite{Lip_reg, LipMLP, PermutoSDF} is a technique used to enforce smoothness by controlling the rate of change of the network's output concerning its inputs.

\begin{comment}
In our work, similarly to \cite{DiffusioNeRF}, we empirically select a combination of term losses, with some modifications on the KL-Divergence loss proposed in Info-NeRF, to constrain the MLP network during the training phase.
\end{comment}
In our work, similarly to \cite{DiffusioNeRF}, we empirically select a combination of term losses to constrain the MLP network during the training phase: we modify the information-theoretic approach of \cite{Info-NeRF} that includes a regularization of neighboring rays distributions, then a smoothness term is adopted to regularize near geometries and we regularize single ray distribution in order to have a specific hitting point on the scene, that reflects real world scenarios.

Additionally, as in \cite{Neuralangelo}, we add an input mask which encourage the learning of finer details only on the latest stages of the training phase.
Finally, we impose Lipshitz regularization on both color and density networks, observing substantial improvements in the overall reconstruction and rendering quality and showing how NeRF benefits from Lipshitz regularization.
Our method avoids the need for pre-training required by similar approaches, while showing promising improvements over the state of the art.

In summary, we present the following contributions:
\begin{itemize}
    \item We propose a modification of the KL-Divergence loss proposed in InfoNeRF.
    \item We select a combination of regularization losses, available on a unified framework, and we validate its effectiveness through ablation studies. 
    \item To our knowledge we are the first to impose Lipshitz regularization on all the network layers on NeRF, recording a performance increase in all the tested scenarios.
\end{itemize}

==> sec/1_intro_OLD.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:relwork}
Novel view synthesis aims to generate images from different viewpoints by utilizing a collection of pre-existing views \cite{deepvoxels, NeuralVolumes, NVSGCD, rgbd, genvs}.
Among the novel view synthesis solutions, NeRF emerged as a result of several factors as the compactness offered by the underlying structure, its domain-agnostic nature and the impressive visual quality offered. Subsequent works managed to improve over the fidelity of rendered images \cite{refnerf, lightfields, DIVeR, rawnerf, blocknerf}, reduce required time \cite{TermiNeRF, donerf, plenoxels, f2nerf} and extend NeRF capabilities and application domain \cite{dnerf, dualNeRF, xnerf, CAMPARI, fignerf, NeRFReN}.\\\\
\textbf{NeRF regularization.}
NeRF models struggle to render novel high quality images when supervised with only few input views during training. 
To lessen the impact of the artifacts introduced by overfitting on training samples previous work focused on the addition of loss terms to provide additional constraints on the model.
In InfoNeRF \cite{Info-NeRF} the entropy of the rays and the KL-divergence between the distribution of close rays are both minimized in order to restrict the range of the prediction of high-density value on the object surface. Similarly to Mip-NeRF 360 \cite{Mip-NeRF360}, distortion loss was introduced to consolidate weights into as small a region as possible when rays intersect a scene object. In RegNeRF and DiffusionNeRF \cite{Reg-NeRF, DiffusioNeRF} rendered patches, which are less likely to appear according to a determined image distribution, are penalized. 
In PixelNerf \cite{PixelNerf}  prior-knowledge acquired from different scenes and global context information are both leveraged by concatenating image features extracted by a Convolutional Neural Network Encoder with the input 3D positions.
In Aug-NeRF \cite{Aug-NeRF} noise is injected into input, feature and output during training to improve the model generalization capabilities.
\textbf{NeuNeural Surface Reconstructionral Surface Reconstruction.}
Implicit functions like signed distance functions (SDFs) \cite{IDR, physg, iron, GO-Surf} and occupancy maps \cite{DVR, NeuralBlox} are best fitted for representing objects on the scene with a defined surface geometry.
Both NeuS and HF-NeuS \cite{NeuS, HF-NeuS} reparametrize the rendering equation used in NeRF to exploit SDFs properties.
In order to increase the training and inference speed and facilitate the learning of high-frequency details, Instant-NSR and Neuralangelo \cite{Instant-NSR, Neuralangelo} exploit the hash grid encoding proposed in Instant-NGP \cite{Instant-NGP}, while PermutoSDF \cite{PermutoSDF} employs a permutohedral lattice to decrease the memory accesses. To recover smoother surfaces in reflective or untextured areas, Neuralangelo and PermutoSDF add a curvature term loss. Additionally Neuralangelo discard values from finer levels of the hash grid encoding to encourage the learning of coarse details on the first training iterations. To prevent the color network overfitting due to the injection of the curvature loss term PermutoSDF employs the Lipschitz constant regularization method proposed by  Liu \etal \cite{LipMLP}.
% In our work we tested some regularization techniques applied on neural surface reconstruction and found out that they can improve the overall prediction quality on NeRF when processing only few images.
In our work we empirica regularization techniques applied on neural surface reconstruction and found out that they can improve the overall prediction quality on NeRF when processing only few images.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_method.tex <==
\section{Method}
\label{sec:method}
The method proposed in this work combines multiple regularization techniques in a unified and flexible framework that helps NeRF generalization in few-shot scenarios. In this section, after providing a preliminary theoretic background, all the combined losses will be described together with the Frequency Encoding Mask and Lipshitz regularization techniques. For each of the elements, all the improvements and modifications will be described in detail to better highlight the main contributions of this work.
\subsection{Preliminaries}
\textbf{Neural Radiance Field.} 
Neural Radiance Field exploits a simple MLP to encode the scene. For each input 3D point and view direction, it outputs the density \(\sigma\) of the point and its color value \(c\). For each pixel, points are sampled on its corresponding camera ray \(r(\mathbf{t})= o + \mathbf{t}d\) and fed to the MLP network. The rendered color is approximated by: 
\begin{equation}
\begin{split}
\begin{gathered}
\label{eq:rendering}
    C(r) = \sum_{i=1}^{N} T_i \left(1 - \exp(-\sigma_i \delta_i)\right) c_i\ ,
\end{gathered}
\end{split}
\end{equation}
where \(\delta_{i} = \mathbf{t_{i+1}}-\mathbf{t_{i}}\) is is the distance between the \(i^{th} \) point and its adjacent sample, \(N\) is the number of samples and the transmittance \(T_{i}\) is computed as:
\begin{equation}
\begin{split}
\begin{gathered}
\label{eq:transmittance}
 T_{i} = \exp\left(-\sum_{j=1}^{i-1} \sigma_j \delta_j\right).
 \end{gathered}
\end{split}
\end{equation}
The rendered pixel color \(C(r)\) can be expressed in terms of a weighted sum of the color values \(C(r) = \sum_{i=1}^{N} w_{i}c_{i}\) where \(w_{i}=T_{i}\alpha_{i}\) with  \(\alpha_{i} = \left(1 - \exp(-\sigma_i \delta_i)\right)\).
The final loss to train the network is the total squared error between
the rendered and true pixel colors:
\begin{equation}
    \mathcal{L}_{RGB}= \sum_{r\in\mathcal{R}} \| C(r) - C^{\ast}(r) \|_2^2.
\end{equation}
\textbf{Multiresolution Hash Encoding.}
In NeRF, a sine-based positional encoding is used to map the 3D point position to a high-dimensional feature vector in order to capture high-frequency details. On the other hand, the multiresolution hash encoding proposed by Müller \etal \cite{Instant-NGP}  adopts multi-resolution grids, achieving a similar result while significantly accelerating training and inference times. This is accomplished by first identifying the cell of the grid containing the point and then assigning the result of the spatial interpolation of the features defined on the corners. As a result, a lightweight MLP can be employed to process the encoded points. Given a input point \(x \in \mathbb{R}^{3}\), its feature vector \(\gamma(x)\in \mathbb{R}^{FL}\) can be expressed as:
\begin{equation}
\begin{split}
\begin{gathered}
\label{eq:hashenc}
 \gamma(x) = \left[\gamma_{1, 1}(x), ..., \gamma_{F, 1}(x), ..., \gamma_{F, L}(x)\right] ,
 \end{gathered}
\end{split}
\end{equation}
where \(F\) is the number of feature dimensions per entry and \(L\) is the number of levels.
To minimize memory usage, each grid corner index is mapped into a hash table that holds its corresponding feature vector. Collisions are limited to finer levels where \((N_{l}+1)^3 > E\), \(N_{l}\) and \(E\) being the resolution at level \(l\) and the maximum number of entries in the hash maps respectively, and they are handled through gradient averaging. This ensures that the results maintain their qualitative comparability to using solely a multi-resolution grid without hash encoding.
\subsection{Regularization Losses}
% We consider an information-theoretic approach that includes a modification of the KL-Divergence loss, then the single ray distribution (Distortion and Full Geometry loss) is regularized also taking into account a smoothness term, called Depth Smoothness loss, to regularize near geometries.\\\\
\begin{comment}
\subsection{Information Theory}
NeRF-based model struggles to reconstruct a 3D scene having only few input views and no knowledge about the scene. The lack of information due to insufficient viewpoints may bring to inconsistency of the scene and degeneracy during training. One way to regularize NeRF can be to use an information-theoretic approach \cite{Info-NeRF} in which we focus on the KL-Divergence formulation (KL-Divergence Loss).\\\\
\end{comment}
\textbf{KL-Divergence Loss.}
When dealing with few training views, the model struggles to generalize to unseen views. 
As 3D scenes exhibits piece-wise smooth surfaces, we enforce similar distributions of weight values among neighbouring rays.
In a different fashion from \cite{Info-NeRF}, we compute the normalized weight distribution $p(\textbf{r})$, defined as:
% For this reason, it's preferable to have consistent distributions among neighbouring rays: in a different way from \cite{Info-NeRF}, we compare the normalized weight distribution $p(\textbf{r})$ defined as

\begin{equation}
\label{eq:probweight}
    p(\textbf{r}_i) = \frac{w_i}{\sum_j w_i} = \frac{T_i \alpha_i}{\sum_j T_j \alpha_j}.
\end{equation}

Given an observed ray $\textbf{r}$, we sample another neighbouring ray $\hat{\textbf{r}}$ minimizing the KL-Divergence ($D_{KL}$) between their weight distribution. The corresponding loss is defined as follows:
\begin{equation}
\label{eq:KL}
\begin{split}
\begin{gathered}
    \mathcal{L}_{KL} = D_{KL}\bigg(  P(\textbf{r}) || P(\hat{\textbf{r}}) \bigg) \\
    = \sum_{i=1}^N p(\textbf{r}_i) \log \frac{p(\textbf{r}_i)}{p(\hat{\textbf{r}}_i)} .
\end{gathered}
\end{split}
\end{equation}
% The choice of the neighbouring ray $\hat{\textbf{r}}$ can be done in two ways: by slightly rotating the camera pose of the ray $\textbf{r}$ or choosing one of the possible adjacent rays (defined as near pixels). In our implementation, we deviate from the original contribution \cite{Info-NeRF} by choosing the second option. After sampling uniformly at random one of the four adjacent rays for each training ray, we compute $\mathcal{L}_{KL}$.\\\\

In our implementation, we deviate from the original implementation \cite{Info-NeRF} where $\hat{\textbf{r}}$ is obtained by slightly rotating the camera pose, generating the ray $\textbf{r}$ by choosing one of the possible adjacent pixel rays. After sampling uniformly at random one of the four adjacent rays for each training ray, we compute $\mathcal{L}_{KL}$.\\\\
% The choice of the neighbouring ray $\hat{\textbf{r}}$ can be done in two ways: by slightly rotating the camera pose of the ray $\textbf{r}$ or choosing one of the possible adjacent rays (defined as near pixels). In our implementation, we deviate from the original contribution \cite{Info-NeRF} by choosing the second option. After sampling uniformly at random one of the four adjacent rays for each training ray, we compute $\mathcal{L}_{KL}$.\\\\
%\subsection{Geometry and Scene Regularization}
\textbf{Distortion and Full Geometry Loss.} A common problem of NeRF is the presence of "floaters", disconnected regions of dense space, usually located close to the camera planes, which cause the presence of blurry clouds artifacts on images rendered from novel views.
Previous works \cite{Mip-NeRF360, DiffusioNeRF} showed that those artifacts can be removed by adding a loss term $\mathcal{L}_{dist}$ that takes into account the distances $t_i$ and weights $w_i$ of the $N$ points sampled on the rays:
\begin{equation}
    d(r) = \frac{\sum_{i=1}^Nw_it_i}{\sum_{i=1}^Nw_i} 
\end{equation}
of each ray. Thus, the $\mathcal{L}_{dist}$ loss can be written as:
\begin{equation}
    \label{eq:dist}
    \begin{split}
    \begin{gathered}
    \mathcal{L}_{dist} =  \frac{1}{d(r)} \Bigg( \sum_{i,j}w_iw_k\left| \frac{t_i+t_{i+1}}{2} - \frac{t_j+t_{j+1}}{2}\right| \\
    + \frac{1}{3} \sum_{i=1}^Nw_{i}^{2}(t_{i+1}-t_i)  \Bigg),
    \end{gathered}
    \end{split}
\end{equation}
where the depth factor penalizes dense regions near the camera. The first term minimizes the weighted distances between all pairs of interval midpoints and the second term minimizes the weighted size of each individual interval. In this way, weights on the ray are encouraged to be as compact as possible by pulling distant intervals towards each other, consolidating weights into a single interval or a small number of nearby intervals and minimizing the width of each interval.

Since \cref{eq:dist} considers all possible intervals for each ray we consider only a subset over the total number of sampled rays on which we compute the loss to reduce the total load.
%In \cref{eq:dist}, all possible intervals for each ray are considered. In practice, the total combination of all $(i,j)$ would drastically increase the amount of memory required. To reduce the total load, we consider only a subset over the total number of sampled rays on which we compute the loss.

Furthermore, a normalization loss term $\mathcal{L}_{fg}$ is considered, following \cite{DiffusioNeRF}, that encourages the weights to sum to unit, as the ray is expected to be fully absorbed by the scene geometry in real scenes:
\begin{equation}
    \mathcal{L}_{fg} =  \left(  1-\sum_{i=1}^Nw_i  \right)^2,
\end{equation}

In addition \(\mathcal{L}_{fg}\) enforce \(\mathcal{L}_{KL}\) by driving the model to treat the weights \(w_{i}\) as probabilities, \(p(\textbf{r}_i) \approx w_{i}\) (See \cref{eq:probweight}).\\\\
\textbf{Depth Smoothness Loss.}
% Starting from the prior that real-world geometries tend to be piece-wise smooth, for example flat surfaces, this knowledge can be added in the model encouraging depth smoothness during the training phase.\\
Similarly to KL-Divergence loss, the depth smoothness constraint encourages smooth surfaces, however, while the former term requires similarity between the compared distributions, the latter term only computes the difference between the expected depth values.
As in \cite{Reg-NeRF}, given the estimate depth $d(r)$ of a pixel ray and a patch of size $S_{patch}$, the depth smoothness constraint is defined as follows:
% Starting from the prior that real-world geometries of the scenes tend to be piece-wise smooth, for example flat surfaces, this knowledge can be added in the model encouraging depth smoothness during the training phase. As done in the previous work \cite{Reg-NeRF}, given the estimate depth $d(r)$ of a ray (that define a specific pixel) and a patch size $S_{patch}$, the depth smoothness constraint is defined as follows:
\begin{equation}
    \begin{split}
    \begin{gathered}
    \mathcal{L}_{ds} = \sum_{p\in P}\sum_{i,j=1}^{S_{patch}-1} \Bigg( \big( d(r_{ij})-d(r_{i+1j})\big)^2 \\
    +\big( d(r_{ij})-d(r_{ij+1}) \big)^2 \Bigg),
    \end{gathered}
    \end{split}
\end{equation}
where $P$ is the set of all the rendered patches, $r_{ij}$ is the ray passing through the pixel $(i,j)$ of patch $p$. 
% In order to compute this loss term is necessary to sample rays through patches instead of sampling them at random, otherwise the depth smoothness prior would not hold anymore because rays could be far away from each other.

\subsection{Encoding Mask}
% One of the problem of neural rendering with few-shot is that NeRF tries to learn the geometry and appearance of the scene given only few 2D input views. It's common that, during training, NeRF overfits on these input views, bringing the 3D reconstruction to poor quality and lots of artifacts.

% One of the reasons behind this problem is that the training is biased toward the high-frequency components of the scene. High-frequency enables fast convergence, but over-fast convergence impedes NeRF to learn good low-frequency information. Especially when dealing with few views, NeRF is even more sensitive to noise since there are fewer images to learn a coherent geometry, and so it is more prone to overfit.

% Our implementation uses hash-encoding (as described in the Instant-NGP implementation \cite{Instant-NGP}) to encode the sampled point used as input to the MLP network. The main idea is to use a masked encoding during training: taking inspiration from \cite{Free-NeRF, Neuralangelo}, we use a masked hash-encoding that regularize the hash-encoding instead of the classic positional-encoding. Given a certain length $l=L\cdot F$ of the resulting hash-encoding given by \ref{eq:hashenc}, a mask $m$ that "deactivate" some features is applied
% \begin{equation}
%     m= [1_{1},...1_{\llbracket l\cdot x \rrbracket},0,...0_{l}],
% \end{equation}
% where $x$ is the ratio of features to keep active. The resulting feature vector given in  input to the MLP network will be the element-wise product $\gamma \odot m$.

% The points are encoded starting from coarsest to finest resolution in order to learn high-frequency details, but training NeRF with high-frequency resolution features from the beginning of the iterations may bring training to diverge. The ratio $x$ is set in such a way to keep the coarsest features during the initial phase of the training and it will progressively include the remaining features until the total length of the encoded point is reached.

% The same reasoning can be applied to a general input of an MLP in order to lower the capacity of the network at the beginning. In fact, this regularization can be done for inputs of both sigma and color MLP, in which different embeddings are given to the network (hash-encoding for sigma and sphere harmonics-encoding for color network).
% One of the problem of neural rendering with few-shot is that NeRF tries to learn the geometry and appearance of the scene given only few 2D input views. It's common that, during training, NeRF overfits on these input views, bringing the 3D reconstruction to poor quality and lots of artifacts.
Input encoding allows the preservation of high-frequency details \cite{NeRF}, however, when only few images are available, the network is more sensitive to noise. In this scenario, high-frequency components exacerbate the problem preventing the network to explore more in depth low-frequency information and consequently learning a coherent geometry.
As in \cite{Free-NeRF, Neuralangelo}, we use a mask to filter out high frequency components of the input in early iterations in order to let the network focus on robust low-frequency information. Given the length $l=L\cdot F$ of the resulting hash-encoding given by \cref{eq:hashenc}, the mask $m$ is defined as:
\begin{equation}
    m= [1_{1},...1_{\llbracket l\cdot x \rrbracket},0,...0_{l}],
\end{equation}
where $x$ is the ratio of features to keep active. The resulting feature vector given in  input to the MLP network will be the element-wise product $\gamma \odot m$.
The ratio $x$ is set to keep only the coarsest features during the initial phase of the training and progressively including the remaining features.
In our implementation we apply Instant-NGP multi-hash encoding on input positions and sphere harmonics encoding on the view directions. The progressive mask can be used on both inputs in order to filter high-frequency terms on early training iterations.

% Additionally, we add the option to apply the mask to filter the sphere harmonics encoding applied on the view directions fed to the color network.

\subsection{Lipshitz Network}
We define $f_\theta(x,t)$ the function representing the implicit shape, expressed by means of a neural network, where $\theta = \{W_i,b_i\}$ is the set of parameters containing weights $W_i$ and biases $b_i$ of each layer $l_{i}$ of the network.

\begin{comment}
In order to have a meaningful representation of the shape, the neural network should be smooth with respect to its latent space.\\
\end{comment}
% Lipshitz regularization penalize $f_\theta$ based on network parameters
A function is called Lipshitz continuous if there exist a constant $k\geq0$ such that: 
\begin{equation}
\label{eq_lipshitz}
    \|f_\theta(x_0) - f_\theta(x_1)\| \leq k \|x_0 - x_1\| ,
\end{equation}
for all possible inputs $x_0$, where $k$ is called the Lipshitz constant which bounds how fast the function $f_\theta$ can change. 
% The key idea is to consider the Lipshitz constant as a learnable parameter and minimize it, instead of fixing it to a certain predefined value.

\begin{comment}
This method requires to determine a matrix $p$-norm and add a weight normalization in the network. For the matrix norm, the choice done is to use the $\inf$-norm (also called maximum norm)
\begin{equation}
    \|W\|_{\infty} = \max_{i}{\sum_{j}{|w_{ij}|}}
\end{equation}
due to its efficiency in the resulting weight normalization.
\end{comment}
We employ the regularization method proposed in \cite{LipMLP}, which was already used by PermutoSDF \cite{PermutoSDF} on the color network to balance out the effect introduced by the curvature regularization applied on the SDF network. However, differently from PermutoSDF we apply the regularization on both NeRF density and color networks, recording an increase in performance w.r.t the vanilla MLP network.
% A previous work \cite{Lipshitz} provides a framework for Lipshitz regularization that is also used in PermutoSDF \cite{PermutoSDF} in the color network. 
Given the trainable Lipshitz bound $k_i$ associated to layer $l_{i}$
% , a Lipshitz weight normalization layer is added for each layer $y = \sigma(W_i x + b_i)$ of an MLP network.
the normalization scheme is described as:
\begin{equation}
    \begin{split}
    \begin{gathered}
    y = \sigma(\hat{W_i} x + b_i)   \\
    \hat{W_i} = f_n(W_i, \ln(1+e^{k_i})),
    \end{gathered}
    \end{split}
\end{equation}
where $f_n$ is a normalization function and $\ln(1+e^{k_i})$ enables to avoid negative values for $k_i$. The normalization scales each row of $W_i$ to have an absolute value row-sum less or equal to $\ln(1+e^{k_i})$ in order to satisfy \cref{eq_lipshitz}.

% As mentioned before, PermutoSDF uses only the normalization scheme in the color network for Signed Distance Function, while in our implementation this regularization is introduced in both NeRF density and color MLP networks. Furthermore, PermutoSDF considers Lipshitz network in order to compute an additional loss. Instead, we prove that the Lipshitz network itself bring a regularization effect that increase the performance w.r.t the classic MLP network.\\


\subsection{Overall Method}
Our method is a combination of the previously described regularization in terms of losses and network structure, hence the term \textit{Combi-NeRF}. Thus, we can write the final loss as:
%\begin{equation}
%    \mathcal{L} = \mathcal{L}_{RGB}+\lambda_{dist}\cdot\mathcal{L}_{dist}+\lambda_{fg}\cdot\mathcal{L}_{fg}+\lambda_{ds}\cdot \mathcal{L}_{ds}+\lambda_{KL}\cdot \mathcal{L}_{KL},
%\end{equation}
\begin{equation}
    \begin{split}
        \begin{gathered}
        \mathcal{L} = \mathcal{L}_{RGB}+\lambda_{dist}\cdot\mathcal{L}_{dist}+\lambda_{fg}\cdot\mathcal{L}_{fg}\\+\lambda_{ds}\cdot \mathcal{L}_{ds}+\lambda_{KL}\cdot \mathcal{L}_{KL} ,
        \end{gathered}
    \end{split}
\end{equation}
where $\lambda$ are the hyperparameters controlling the contribution of each loss.
In addition our method includes \textbf{Lipshitz} regularization and the \textbf{Encoding Mask} technique.

The proposed Combi-NeRF offers a unified implementation of all the regularization techniques described above, outperforming current state-of-the-art methods on few-shot scenarios as demonstrated in the following experimental section.

==> sec/4_experiments.tex <==
\definecolor{White}{rgb}{1,1,1}
\definecolor{LightCyan}{rgb}{0.74,0.83,0.9}

\section{Experiment} 
\label{sec:experiment}
In this section we show the dataset and metrics we use for the experiments, we provide relevant details about our implementation and we show quantitative and qualitative comparisons made against the state-of-the art methods. Finally, an ablation study is made to evaluate the contribution of the components which forms Combi-NeRF.

\subsection{Setup}

\textbf{Dataset.}
Our experiments includes the LLFF dataset \cite{LLFF} and NeRF-Synthetic dataset \cite{NeRF} under few-shot settings. LLFF is composed by 8 complex scenes, representing real-world scenarios, with 20-62 images for each scene captured with an handled camera. Instead, NeRF-Synthetic is composed by 8 synthetic scenes with view-dependent light transport effects, in which each scene is composed by 100 training images and 200 test images.

We evaluate LLFF on 3/6/9 input views, adhering to Reg-NeRF's \cite{Reg-NeRF} protocol, while in NeRF-Synthetic we train 8 views and test 25 views following Diet-NeRF \cite{Diet-NeRF}.\\\\
\textbf{Metrics.}
To evaluate the performance of our implementation against the SOTA methods, we use 3 different metrics: peak signal-to-noise ratio (PSNR), structural similarity index measure (SSIM) \cite{SSIM} and learned perceptual image patch similarity (LPIPS) \cite{LPIPS}. Furthermore, we also take into consideration the geometric mean of $\text{MSE}=10^{-\text{PSNR}/10}$, $\sqrt{1-\text{SSIM}}$ and LPIPS following \cite{Reg-NeRF}, in order to have an easier and unified comparison.\\\\
\textbf{Implementation Details.}
For our experiments, we use the torch-ngp \cite{torch-NGP} implementation of Instant-NGP \cite{Instant-NGP} as base code, and then we develop our method on top of it obtaining a unified and unique implementation that includes all the contribution shown in the previous section.

For the LLFF dataset we set $\lambda_{dist} = 0$ for the first 1000 iteration and then $\lambda_{dist} = 2\cdot10^{-5}$ until the end and $\lambda_{fg} = 10^{-4}$, $\lambda_{KL} = 10^{-5}$, $\lambda_{ds} = 0.1$ and $S_{patch} = 4$, while we use the encoding mask only on the density network in which $x$ saturates after 90\% of the total iterations. In the NeRF-Synthetic dataset we set $\lambda_{dist} = 0$ for the first 1000 iteration and then $\lambda_{dist} = 2\cdot10^{-3}$ until the end and $\lambda_{fg} = 10^{-3}$, $\lambda_{KL} = 10^{-5}$, $\lambda_{ds} = 0.01$ and $S_{patch} = 4$, $x$ saturates after 20\% of the total iterations. We also set the number sampled rays for each iteration to 4096 and 7008 and  1the number of levels for the Instant-NGP hash-encoding to 16 and 32 for LLFF and NeRF-Synthetic respectively.

\subsection{Comparison}
We compare the performance achieved with our implementation against the state-of-the-art methods in the few-shot scenario. In LLFF we consider Reg-NeRF \cite{Reg-NeRF}, Free-NeRF \cite{Free-NeRF} and DiffusioNeRF \cite{DiffusioNeRF}, while in NeRF-Synthetic we take into account DietNeRF \cite{Diet-NeRF} and Free-NeRF.\\\\
\textbf{LLFF Dataset.}
\begin{table*}[t] \centering
    \resizebox{\textwidth}{!}{
    \Huge
    \rowcolors{2}{LightCyan}{White}
        \begin{tabular}{p{10cm}|*{3}{c}|*{3}{c}|*{3}{c}|*{3}{c}}
        \toprule
        & \multicolumn{3}{c}{PSNR $\uparrow$} 
                               & \multicolumn{3}{c}{SSIM $\uparrow$} 
                               & \multicolumn{3}{c}{LPIPS $\downarrow$} 
                               & \multicolumn{3}{c}{Average $\downarrow$}  \\
                               & 3-view & 6-view & 9-view
                               & 3-view & 6-view & 9-view 
                               & 3-view & 6-view & 9-view 
                               & 3-view & 6-view & 9-view \\
        \midrule
        Vanilla    &  17.71 & 22.03 & 24.21 & 0.544 & 0.738 & 0.811 & 0.303 & 0.149 & 0.101 & 0.155 & 0.081 & 0.057\\
        Reg-NeRF    &  19.08 & 23.10 & 24.86 & 0.587 & 0.760 & 0.820 & 0.336 & 0.206 & 0.161 & 0.146 & 0.086 & 0.067\\    
        Free-NeRF    &  19.63 & 23.73 & 25.13 & 0.612 & 0.779 & 0.827 & 0.308 & 0.195 & 0.160 & 0.134 & 0.075 & 0.064 \\        
        Diff-NeRF     &  19.88 & \textbf{24.28} & 25.10 & 0.590 & 0.765 & 0.802 & 0.192 & \textbf{0.101} & \textbf{0.084} & 0.118 & 0.071 & 0.060\\
        %Ours no KL-D    &  20.27 & 24.01 & 25.14 & 0.683 & \textbf{0.806} & \textbf{0.841} & 0.194 & 0.105 & \textbf{0.083} & 0.103 & \textbf{0.060} & \textbf{0.049} \\
        \midrule
            Combi-NeRF       &  \textbf{20.37} & 23.99 & \textbf{25.15} & \textbf{0.686} & \textbf{0.805} & \textbf{0.841} & \textbf{0.191} & 0.106 & \textbf{0.084} & \textbf{0.101} & \textbf{0.060} & \textbf{0.049} \\
        \bottomrule
        \end{tabular}
    }
    \caption{NeRF SOTA comparison on LLFF dataset with 3/6/9 input views.}
    \label{tab:table8}
\end{table*}
% 3-views
\begin{figure*}[t] \centering
    \makebox[0.195\textwidth]{Vanilla}
    \makebox[0.195\textwidth]{RegNeRF}
    \makebox[0.195\textwidth]{FreeNeRF}
    \makebox[0.195\textwidth]{Combi-NeRF}
    \makebox[0.195\textwidth]{GT}
    \\
    \includegraphics[width=0.195\textwidth]{images/Vanilla/fern/ngp_ep3000_0003_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/RegNeRF/fern3/color_002.png}
    \includegraphics[width=0.195\textwidth]{images/FreeNeRF/fern3/color_002.png}
    \includegraphics[width=0.195\textwidth]{images/fern/ngp_ep3000_0003_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/GT/fern/image016.png}
    \\
    \includegraphics[width=0.195\textwidth]{images/Vanilla/horns/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/RegNeRF/horns3/color_003.png}
    \includegraphics[width=0.195\textwidth]{images/FreeNeRF/horns3/color_003.png}
    \includegraphics[width=0.195\textwidth]{images/horns/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/GT/horns/DJI_20200223_163047_307.png}
    \\
    \includegraphics[width=0.195\textwidth]{images/Vanilla/trex/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/RegNeRF/trex3/color_003.png}
    \includegraphics[width=0.195\textwidth]{images/FreeNeRF/trex3/color_003.png}
    \includegraphics[width=0.195\textwidth]{images/trex/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.195\textwidth]{images/GT/trex/DJI_20200223_163611_160.png}
    \caption{Comparison of our Combi-NeRF against RegNeRF, FreeNeRF and our Vanilla on Fern, Horns and Trex scenarios with 3-view setting.} 
    \label{fig:figure1}
\end{figure*}
\begin{figure}[t] \centering
    \makebox[0.15\textwidth]{FreeNeRF}
    \makebox[0.15\textwidth]{Combi-NeRF}
    \makebox[0.15\textwidth]{GT}
    \\
    \includegraphics[width=0.15\textwidth]{images/FreeNeRF/room9/color_005_border.png}
    \includegraphics[width=0.15\textwidth]{images/room/ngp_ep1334_0006_rgb_border.png}
    \includegraphics[width=0.15\textwidth]{images/GT/room/DJI_20200226_143948_113_border.png}
    \\
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.1\textwidth]{images/zoom/freeroom_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.1\textwidth]{images/zoom/ourroom_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.1\textwidth]{images/zoom/gtroom_border.png}}
    \\[-0.1em]
    \makebox[\columnwidth]{\small (a) 9-view Room dataset} 
    \\[0.5em]
    \includegraphics[width=0.15\textwidth]{images/FreeNeRF/orchids6/color_001_border.png}
    \includegraphics[width=0.15\textwidth]{images/orchids/ngp_ep1667_0002_rgb_border.png}
    \includegraphics[width=0.15\textwidth]{images/GT/orchids/image008_border.png}
    \\
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.08\textwidth]{images/zoom/freeorchids_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.08\textwidth]{images/zoom/ourorchids_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.08\textwidth]{images/zoom/gtorchids_border.png}}
    \\[-0.1em]
    \makebox[\columnwidth]{\small (b) 6-view Orchids dataset.} 
    \\[0.5em]
    \includegraphics[width=0.15\textwidth]{images/FreeNeRF/leaves3/color_003_border.png}
    \includegraphics[width=0.15\textwidth]{images/leaves/ngp_ep3000_0004_rgb_border.png}
    \includegraphics[width=0.15\textwidth]{images/GT/leaves/image024_border.png}
    \\
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.07\textwidth]{images/zoom/freeleaves_part-0_border.png}
        \hspace{0.2pt}
        \includegraphics[width=0.07\textwidth]{images/zoom/freeleaves_part-1_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.07\textwidth]{images/zoom/ourleaves_part-0_border.png}
        \hspace{0.2pt}
        \includegraphics[width=0.07\textwidth]{images/zoom/ourleaves_part-1_border.png}}
    \makebox[0.15\textwidth]{%
        \includegraphics[width=0.07\textwidth]{images/zoom/gtleaves_part-0_border.png}
        \hspace{0.2pt}
        \includegraphics[width=0.07\textwidth]{images/zoom/gtleaves_part-1_border.png}}
    \\[-0.1em]
    \makebox[\columnwidth]{\small (c) 3-view Leaves dataset.} 
    \\[0.5em]
    \caption{Comparison of Combi-NeRF against FreeNeRF with 3/6/9 input views.} 
    \label{fig:figure4}
\end{figure}
\begin{comment}
% 3-views
\begin{figure*}[t] \centering
    \makebox[0.23\textwidth]{Fern}
    \makebox[0.23\textwidth]{Horns}
    \makebox[0.23\textwidth]{Trex}
    \makebox[0.23\textwidth]{Leaves}
    \\
    \raisebox{0.1\height}{\makebox[0.01\textwidth]{\rotatebox{90}{\makecell{Combi-NeRF}}}}
    \includegraphics[width=0.23\textwidth]{images/fern/ngp_ep3000_0003_rgb.png}
    \includegraphics[width=0.23\textwidth]{images/horns/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.23\textwidth]{images/trex/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.23\textwidth]{images/leaves/ngp_ep3000_0004_rgb.png}
    \\
    \raisebox{0.1\height}{\makebox[0.01\textwidth]{\rotatebox{90}{\makecell{FreeNeRF}}}}
    \includegraphics[width=0.23\textwidth]{images/FreeNeRF/fern3/color_002.png}
    \includegraphics[width=0.23\textwidth]{images/FreeNeRF/horns3/color_003.png}
    \includegraphics[width=0.23\textwidth]{images/FreeNeRF/trex3/color_003.png}
    \includegraphics[width=0.23\textwidth]{images/FreeNeRF/leaves3/color_003.png}
    \\
    \raisebox{0.1\height}{\makebox[0.01\textwidth]{\rotatebox{90}{\makecell{RegNeRF}}}}
    \includegraphics[width=0.23\textwidth]{images/RegNeRF/fern3/color_002.png}
    \includegraphics[width=0.23\textwidth]{images/RegNeRF/horns3/color_003.png}
    \includegraphics[width=0.23\textwidth]{images/RegNeRF/trex3/color_003.png}
    \includegraphics[width=0.23\textwidth]{images/RegNeRF/leaves3/color_003.png}
    \\
    \raisebox{0.1\height}{\makebox[0.01\textwidth]{\rotatebox{90}{\makecell{Combi-NeRF}}}}
    \includegraphics[width=0.23\textwidth]{images/fern/ngp_ep3000_0003_depth.png}
    \includegraphics[width=0.23\textwidth]{images/horns/ngp_ep3000_0004_depth.png}
    \includegraphics[width=0.23\textwidth]{images/trex/ngp_ep3000_0004_depth.png}
    \includegraphics[width=0.23\textwidth]{images/leaves/ngp_ep3000_0004_depth.png}
    \caption{Comparison of our Combi-NeRF against RegNeRF and FreeNeRF on Fern, Horns, Trex and Leaves scenarios with 3-view setting.} 
    \label{fig:figure1}
\end{figure*}
\end{comment}
In this collection of real world complex scenes, we can observe that NeRF heavily overfits on training images when only a few of them are used as input. With our multiple combination of regularization, we are able to achieve better results with respect to SOTA methods. In \cref{tab:table8} are shown the quantitative results under 3/6/9 training images. For 3 and 9 views, our implementation outperforms the other methods in all the metrics. With 6 views, DiffusioNeRF achieves a better LPIPS score, however our method scores higher on the average.

In addition, we can observe that the vanilla implementation achieve better average score in 9 views setting with respect to all the other examined SOTA methods, excluding our proposed solution, and in 6 views setting with respect to Reg-NeRF. However, in 3 view setting performances heavily degrade.
%We deduce that the vanilla implementation, 
% It's interesting to notice that the experiments made with the vanilla implementation achieve better average score in 9 views setting with respect to all the other SOTA methods, and in 6 views setting with respect to Reg-NeRF. This means that NeRF with hash-encoding is able to obtain very good performance even without regularization, having enough images.

Qualitative results are shown in \cref{fig:figure1}. Combi-NeRF is able to reconstruct better high-frequency details maintaining the geometry of the scene. Other methods generates lots of artifacts, like in "Fern" scene, and they struggle to reconstruct the background. In "Horns", the environment is noisy in RegNeRF and FreeNeRF while it become sharper in Combi-NeRF. We also notice that some fine details like the stair handrail of "Trex" scene are preserved.

In \cref{fig:figure4} we compare Combi-NeRF with FreeNeRF. In "Room" with 9-view setting, the near part of the table get deformed while in Combi-NeRF some details on the floor are still visible. In "Orchids" with 6-view setting, Combi-NeRF is able to render more high-frequency details, for example stripes in the orchid petals (\cref{fig:figure4}). In "Leaves" with 3-view setting, the central leaf rendered in FreeNeRF contains some artifacts and in general, even in this case, Combi-NeRF is able to reconstruct better high-frequency details.

The quantitative evaluation results for the other methods in \cref{tab:table8}, and the corresponding qualitative results in \cref{fig:figure1} and \cref{fig:figure4} are taken from the respective original papers.\\\\
\textbf{NeRF-Synthetic Dataset.}
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\rowcolors{2}{LightCyan}{White}
\begin{tabular}{c | c c c}
\toprule
NeRF-Synthetic 8-views & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\
\midrule
Vanilla  & 22.335 & 0.845 & 0.144    \\
DietNeRF & 23.147 & 0.866 & 0.109 \\
DietNeRF, $\mathcal{L}_{MSE}$ ft & 23.591 & 0.874 & 0.097    \\
Free-NeRF & 24.259 & \textbf{0.883} & 0.098    \\
%Ours with KL-D(near pose) & 24.360 & \textbf{0.883} & \textbf{0.088}    \\
\midrule
Combi-NeRF & \textbf{24.394} & \textbf{0.883} & \textbf{0.088}    \\
\bottomrule
% old Dist+Fg+KL-D+Patch depth Loss+lipshitz+Encoding mask & \textbf{24.314} & \textbf{0.883} & \textbf{0.086}    \\
\end{tabular}
}
\caption{NeRF SOTA comparison on NeRF-Synthetic dataset with 8 input views. "$\mathcal{L}_{MSE}$ ft" is the fine-tuned version of DietNeRF.}
\label{tab:table7}
\end{table}
\begin{figure}[t] \centering
    \makebox[0.11\textwidth]{Vanilla}
    \makebox[0.11\textwidth]{}
    \makebox[0.11\textwidth]{Combi-NeRF}
    \makebox[0.11\textwidth]{}
    \\
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/drums/ngp_ep0150_0012_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/drums/ngp_ep0150_0012_depth.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/drums/ngp_ep0350_0012_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/drums/ngp_ep0350_0012_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/ship/ngp_ep0100_0008_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/ship/ngp_ep0100_0008_depth.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/ship/ngp_ep1150_0008_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/ship/ngp_ep1150_0008_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/materials/ngp_ep0350_0007_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/materials/ngp_ep0350_0007_depth.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/materials/ngp_ep0700_0007_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/materials/ngp_ep0700_0007_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/ficus/ngp_ep0100_0007_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/ficus/ngp_ep0100_0007_depth.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/ficus/ngp_ep0250_0007_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/ficus/ngp_ep0250_0007_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/hotdog/ngp_ep0100_0020_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/vanilla/hotdog/ngp_ep0100_0020_depth.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/hotdog/ngp_ep1250_0020_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/synthetic/hotdog/ngp_ep1250_0020_depth.png}
    \caption{Comparison of Combi-NeRF against our Vanilla method in Drums, Ship, Materials, Ficus and Hotdog scenarios.} 
    \label{fig:figure5}
\end{figure}

This dataset contains synthetic renderings of objects exhibiting high-frequency geometric details and reflective effects.
In \cref{tab:table7} we show the quantitative results. Our implementation outperforms the other SOTA methods with respect to PSNR and LPIPS metrics, while achieving the same result on SSIM. In general we are able to obtain the best quantitative results.
Our method perform better on scenes like "Lego", "Mic", "Ficus", while "Materials" represents the most challenging scenario due to the presence of strong view-dependent reflection. 
% but the more challenging scene are the one with strong view-dependent reflection such as "Materials". Instead, more detailed scenes like "Lego", "Mic", "Ficus" are well reconstructed and keep high frequency information. Analyzing the results from Instant-NGP, we encounter a similar trend over the scenes, hence this could be an explanation of the previous fact since we use their encoding. Evaluation results for \cref{tab:table7} are taken from the respective papers.

In \cref{fig:figure5} we show qualitative results of Combi-NeRF in different scenes. The reconstructed depth is more consistent, presenting less artifacts. Rendered images are far less noisy with respect to the ones rendered by the Vanilla version and colors are preserved as can be seen in "Hotdog" and in "Ficus" where the color of the leaves is brown instead of green.\\
The quantitative evaluation results for the other methods in \cref{tab:table7} are taken from the respective papers.

\subsection{Ablation Study}
In this section we show the contribution of some of the components of our implementation. The choice was made empirically based on various intermediate test we made for the study of the combinations of these forms of regularization.

We ablate our method under 3 view setting on LLFF dataset, while we use 8 view setting for NeRF-Synthetic dataset. For this ablation, we use the same parameters of the experiments previously described.\\\\
\textbf{LLFF dataset.}
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\rowcolors{2}{LightCyan}{White}
\begin{tabular}{c | c c c | c}
\toprule
LLFF 3-views & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Average $\downarrow$  \\
\midrule
Vanilla    &  17.71 & 0.544 & 0.303 & 0.155 \\
L & 18.74 & 0.608 & 0.249 & 0.130     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg} $ & 17.93 & 0.554 & 0.288 & 0.151     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$ ($S_{patch}=4$) & 19.10 & 0.608 & 0.249 & 0.128     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$ & 19.50 & 0.626 & 0.237 & 0.122     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$+L & 20.09 & 0.674 & 0.198 & 0.105     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$+L+EM & 20.27 & 0.683 & 0.194 & 0.103     \\
Combi-NeRF$^{\sharp}$ & 19.52 & 0.637 & 0.236 & 0.119     \\
\midrule
Combi-NeRF  &  \textbf{20.37} & \textbf{0.686} & \textbf{0.191} & \textbf{0.101}  \\
\bottomrule
\end{tabular}
}
\caption{Ablation on LLFF dataset with 3-view setting. Lipshitz is defined as L and Encoding Mask is defined as EM. We set $S_{patch}=4$ when $\mathcal{L}_{ds}$ is included, otherwise we write it explicitly. We call Combi-NeRF$^{\sharp}$ our method using Lipshitz only in the color network.}
\label{tab:table6}
\end{table}
\begin{figure}[t] \centering
    \makebox[0.11\textwidth]{Combi-NeRF$^{\sharp}$}
    \makebox[0.11\textwidth]{}
    \makebox[0.11\textwidth]{Combi-NeRF}
    \makebox[0.11\textwidth]{}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_color/orchids/ngp_ep3000_0002_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_color/orchids/ngp_ep3000_0002_depth.png}
    \includegraphics[width=0.11\textwidth]{images/orchids/ngp_ep3000_0002_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/orchids/ngp_ep3000_0002_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_color/fortress/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_color/fortress/ngp_ep3000_0004_depth.png}
    \includegraphics[width=0.11\textwidth]{images/fortress/ngp_ep3000_0004_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/fortress/ngp_ep3000_0004_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_color/horns/ngp_ep3000_0005_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_color/horns/ngp_ep3000_0005_depth.png}
    \includegraphics[width=0.11\textwidth]{images/horns/ngp_ep3000_0005_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/horns/ngp_ep3000_0005_depth.png}
    \caption{Qualitative result on the ablation study of LLFF with 3-view setting. We compare our Combi-NeRF with Combi-NeRF$^{\sharp}$ (our method using Lipshitz only in the color network).} 
    \label{fig:figure2}
\end{figure}
In \cref{tab:table6} is shown the ablation on LLFF dataset with 3 view setting. We notice that all the single implementations of our method contributes to the overall performance, with Lipshitz regularization and $\mathcal{L}_{dist}+\mathcal{L}_{fg}$ losses playing a crucial role in improving the overall performance. Applying Lipshitz regularization on both networks allow to further improve the quality of the obtained results. 
% Moreover, it's fundamental to use patch sampling over the rays, as observed in particular for $\mathcal{L}_{dist}+\mathcal{L}_{fg}$ loss.

In \cref{fig:figure2} we show qualitative results of Combi-NeRF using Lipshitz regularization in both sigma and color network against only color network.
% The depth is definitely better reconstructed using Combi-NeRF since we use regularization also in the sigma network.
Combi-NeRF is able to model in a more coherent way the geometry of the scenarios, removing also the blurry effects that characterize the renderings of the implementation using only Lipshitz regularitazion in the color network.\\\\
\textbf{NeRF-Synthetic dataset.}
\begin{table}[t]
\resizebox{\columnwidth}{!}{
\rowcolors{2}{LightCyan}{White}
\begin{tabular}{c | c c c | c}
\toprule
NeRF-Synthetic 8-views & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & Average $\downarrow$  \\
\midrule
Vanilla & 22.34 & 0.845 & 0.144 & 0.073     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$+L & 23.61 & 0.865 & 0.115 & 0.059     \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$+$\mathcal{L}_{KL}^{\dagger}$+L & 22.93 & 0.863 & 0.126 & 0.064   \\
$\mathcal{L}_{dist}$+$\mathcal{L}_{fg}$+$\mathcal{L}_{ds}$+L+EM & 24.04 & 0.871 & 0.105 & 0.056   \\
Combi-NeRF$^{\dagger}$ & 24.36 & \textbf{0.883} & \textbf{0.088} & \textbf{0.050}   \\
\midrule
Combi-NeRF & \textbf{24.39} & \textbf{0.883} & \textbf{0.088} & 0.051   \\
\bottomrule
\end{tabular}
}
\caption{Ablation on NeRF-Synthetic dataset with 8-view setting. Lipshitz is defined as L and Encoding Mask is defined as EM. We call $\mathcal{L}_{KL}^{\dagger}$ the KL-Divergence loss presented by InfoNeRF and we call Combi-NeRF$^{\dagger}$ our method using their $\mathcal{L}_{KL}^{\dagger}$.} 
\label{tab:table5}
\end{table}
\begin{figure}[t] \centering
    \makebox[0.11\textwidth]{Combi-NeRF$^{\dagger}$}
    \makebox[0.11\textwidth]{}
    \makebox[0.11\textwidth]{Combi-NeRF}
    \makebox[0.11\textwidth]{}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/lego/ngp_ep0700_0016_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/lego/ngp_ep0700_0016_depth.png}
    \includegraphics[width=0.11\textwidth]{images/lego/ngp_ep0700_0016_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/lego/ngp_ep0700_0016_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/hotdog/ngp_ep0700_0019_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/hotdog/ngp_ep0700_0019_depth.png}
    \includegraphics[width=0.11\textwidth]{images/hotdog/ngp_ep1250_0019_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/hotdog/ngp_ep1250_0019_depth.png}
    \\
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/chair/ngp_ep0650_0014_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/ablation_KL/chair/ngp_ep0650_0014_depth.png}
    \includegraphics[width=0.11\textwidth]{images/chair/ngp_ep0700_0014_rgb.png}
    \includegraphics[width=0.11\textwidth]{images/chair/ngp_ep0700_0014_depth.png}
    \caption{Qualitative result on the ablation study of NeRF-Synthetic with 8-view setting. We compare our Combi-NeRF with Combi-NeRF$^{\dagger}$ (our method using the KL-Divergence presented by InfoNeRF).} 
    \label{fig:figure3}
\end{figure}
In \cref{tab:table5} is shown the ablation on NeRF-Synthetic with 8 view setting. We focused more on $\mathcal{L}_{KL}$, experimenting the implementation of KL-Divergence used in Info-NeRF \cite{Info-NeRF} where they use $\alpha$ instead of $w$ and the rays are sampled through near pose of the camera instead of our near rays setting. 

% We notice that this changing doesn't affect the quantitative performance in this dataset, but still it's a good choice. Anyway, together with all the other components, we reach the best result and this validate our hypothesis that the combination of the presented regularization approaches enable better performance.

In \cref{fig:figure3} we compare qualitative results of Combi-NeRF by changing the implementation of KL-Divergence as mentioned before (Combi-NeRF$^{\dagger}$). While quantitative results remain the same, Combi-NeRF is able to remove most of the artifact generated under the plate of "Hotdog", under the baseline of "Lego" and under the "Chair", indicating an improved reconstruction of the geometry of the objects.

==> sec/5_conclusion.tex <==
\section{Conclusion} 
\label{sec:conclusion}
We have presented Combi-NeRF, a combination of regularization techniques in a single and unified framework. We focus on an information-theoretic approach to regularize neighboring rays distributions, we also take into account the single ray distribution and a smoothness term is adopted to regularize near geometries. Beside these additional loss functions, we consider the network regularization using Lipshitz function and an Encoding Mask to regularize high-frequency components.

Combi-NeRF show impressive results in the quality of the reconstructions and it outperforms the state-of-the-art methods in LLFF and NeRF-Synthetic dataset with few-shot setting. The increasing performance of the combination of multiple regularization techniques is validated through our ablation study that highlights the contribution of Combi-NeRF components and the differences with the previous implementations.

Future work can be done taking into account different dataset and introducing new forms of regularization that could bring better quality reconstruction.
